Dimensionality Reduction for k-Means Clustering and Low Rank Approximation

We show how to approximate a data matrix $\mathbf{A}$ with a much smaller sketch $\mathbf{\tilde A}$ that can be used to solve a general class of constrained k-rank approximation problems to within $(1+\epsilon)$ error. Importantly, this class of problems includes $k$-means clustering and unconstrained low rank approximation (i.e. principal component analysis). By reducing data points to just $O(k)$ dimensions, our methods generically accelerate any exact, approximate, or heuristic algorithm for these ubiquitous problems. For $k$-means dimensionality reduction, we provide $(1+\epsilon)$ relative error results for many common sketching techniques, including random row projection, column selection, and approximate SVD. For approximate principal component analysis, we give a simple alternative to known algorithms that has applications in the streaming setting. Additionally, we extend recent work on column-based matrix reconstruction, giving column subsets that not only `cover' a good subspace for $\bv{A}$, but can be used directly to compute this subspace. Finally, for $k$-means clustering, we show how to achieve a $(9+\epsilon)$ approximation by Johnson-Lindenstrauss projecting data points to just $O(\log k/\epsilon^2)$ dimensions. This gives the first result that leverages the specific structure of $k$-means to achieve dimension independent of input size and sublinear in $k$.

==> error_matrices_app.tex <==
\section{Approximate Constrained Low Rank Approximation}
\label{pcp_application}
In this section, we show that any constrained low rank approximation problem (see Section \ref{subsec:constrained}) can be solved approximately for a matrix $\bv{A}$ by optimizing over a projection-cost preserving sketch of $\bv{A}$. We prove the following lemmas from Section \ref{subsec:app_to_constrained_low_rank}:

\begin{replemma}{sketch_approximation}[Low Rank Approximation via Projection-Cost Preserving Sketches] For any $\bv{A}\in \R^{n\times d}$ and any set $S$ of rank $k$ orthogonal projections, let $\bv{P^*} = \argmin_{\bv{P} \in S} \norm{\bv{A} - \bv{P}\bv{ A}}_F^2$. Accordingly, for any $\bv{\tilde A} \in \mathbb{R}^{n \times d'}$, let $\bv{\tilde P}^* = \argmin_{\bv{P} \in S} \norm{\bv{\tilde A} - \bv{P}\bv{\tilde A}}_F^2$. If $\bv{\tilde A}$ is a rank $k$ projection-cost preserving sketch for $\bv{A}$ with error $\epsilon$, then for any $\gamma \ge 1$, 
if $\norm{\bv{\tilde A} - \bv{\tilde P} \bv{\tilde A}}_F^2 \le \gamma \norm{\bv{\tilde A} - \bv{\tilde P}^* \bv{\tilde A}}_F^2$ 
\begin{align*}
\norm{\bv{ A} - \bv{\tilde P} \bv{ A}}_F^2 \le \frac{(1+\epsilon)}{(1-\epsilon)} \cdot \gamma \norm{\bv{A}-\bv{P^* A}}_F^2.
\end{align*}
\end{replemma}

\begin{proof}

By optimality of $\bv{\tilde P}^*$ for $\bv{\tilde A}$, $\norm{\bv{\tilde A} - \bv{\tilde P^*}\bv{\tilde A}}_F^2 \leq \norm{\bv{\tilde A} - \bv{P^*}\bv{\tilde A}}_F^2$ and thus,
\begin{align}\label{approx1}
\norm{\bv{\tilde A} - \bv{\tilde P}\bv{\tilde A}}_F^2 \le \gamma \norm{\bv{\tilde A} - \bv{P^*}\bv{\tilde A}}_F^2.
\end{align}
Furthermore, since $\bv{\tilde A}$ is projection-cost preserving, the following two inequalities hold:
\begin{align}\label{approx2}
\norm{\bv{\tilde A} - \bv{P^*}\bv{\tilde A}}_F^2  \le (1+\epsilon) \norm{\bv{A} - \bv{P^*}\bv{ A}}_F^2- c,\\
\label{approx3}
\norm{\bv{\tilde A} - \bv{\tilde P}\bv{\tilde A}}_F^2  \ge (1-\epsilon)\norm{\bv{A} - \bv{\tilde P}\bv{A}}_F^2 - c.
\end{align}
Combining \eqref{approx1},\eqref{approx2}, and \eqref{approx3}, we see that:
\begin{align*}
(1-\epsilon)\norm{\bv{ A} - \bv{\tilde P} \bv{ A}}_F^2 - c &\le (1+\epsilon) \cdot \gamma \norm{\bv{A}-\bv{P^* A}}_F^2 - \gamma c\\
\norm{\bv{ A} - \bv{\tilde P} \bv{ A}}_F^2 &\le \frac{(1+\epsilon)}{(1-\epsilon)} \cdot \gamma \norm{\bv{A}-\bv{P^* A}}_F^2,
\end{align*} 
where the final step is simply the consequence of $c \geq 0$ and $\gamma \ge 1$.
\end{proof}

\begin{replemma}{sketch_approximation_improved}[Low Rank Approximation via One-sided Error Projection-Cost Preserving Sketches] For any $\bv{A}\in \R^{n\times d}$ and any set $S$ of rank $k$ orthogonal projections, let $\bv{P^*} = \argmin_{\bv{P} \in S} \norm{\bv{A} - \bv{P}\bv{ A}}_F^2$. Accordingly, for any $\bv{\tilde A} \in \mathbb{R}^{n \times d'}$, let $\bv{\tilde P}^* = \argmin_{\bv{P} \in S} \norm{\bv{\tilde A} - \bv{P}\bv{\tilde A}}_F^2$. If $\bv{\tilde A}$ is a rank $k$ projection-cost preserving sketch for $\bv{A}$ with one-sided error $\epsilon$, then for any $\gamma \ge 1$, 
if $\norm{\bv{\tilde A} - \bv{\tilde P} \bv{\tilde A}}_F^2 \le \gamma \norm{\bv{\tilde A} - \bv{\tilde P}^* \bv{\tilde A}}_F^2$
\begin{align*}
\norm{\bv{ A} - \bv{\tilde P} \bv{ A}}_F^2 \le (1+\epsilon) \cdot \gamma \norm{\bv{A}-\bv{P^* A}}_F^2.
\end{align*}
\end{replemma}
\begin{proof}
Identical to the proof of Lemma \ref{sketch_approximation} except that \eqref{approx3} can be replaced by $\norm{\bv{\tilde A} - \bv{\tilde P}\bv{\tilde A}}_F^2  \ge \norm{\bv{A} - \bv{\tilde P}\bv{A}}_F^2 - c$, which gives  the result when combined with \eqref{approx1} and \eqref{approx2}.
\end{proof}

